An Introduction to Modern Statistical Learning

This work in progress aims to provide a unified introduction to statistical learning, building up slowly from classical models like the GMM and HMM to modern neural networks like the VAE and diffusion models. There are today many internet resources that explain this or that new machine-learning algorithm in isolation, but they do not (and cannot, in so brief a space) connect these algorithms with each other or with the classical literature on statistical models, out of which the modern algorithms emerged. Also conspicuously lacking is a single notational system which, although unfazing to those already familiar with the material (like the authors of these posts), raises a significant barrier to the novice's entry. Likewise, I have aimed to assimilate the various models, wherever possible, to a single framework for inference and learning, showing how (and why) to change one model into another with minimal alteration (some of them novel, others from the literature). Some background is of course necessary. I have assumed the reader is familiar with basic multivariable calculus, probability and statistics, and linear algebra. The goal of this book is certainly not completeness, but rather to draw a more or less straight-line path from the basics to the extremely powerful new models of the last decade. The goal then is to complement, not replace, such comprehensive texts as Bishop's \emph{Pattern Recognition and Machine Learning}, which is now 15 years old.

==> figures.tex <==
% FIGURES FOR IMSL

%---------------------------- NECESSARY DEFINITIONS --------------------------%
\usepackage{psfrag}
\def\EXT{eps}
%-----------------------------------------------------------------------------%
\tikzset{latent/.append style={minimum size=0.8cm}}
\tikzset{obs/.append style={minimum size=0.8cm}}
    


\newcommand{\FigMixtureOfGaussians}{
	\begin{figure}[!t]
		\newcommand{\figwidth}{0.35\textwidth}%
		\newcommand{\figheight}{0.35\textwidth}%
		\provideboolean{CLEANXAXIS}%
		\setboolean{CLEANXAXIS}{true}%
		\provideboolean{CLEANYAXIS}%
		\setboolean{CLEANYAXIS}{true}%
		\subfloat[][]{
			\centering
			\label{subfig:cluster}
			\ifthenelse{\boolean{INCLFIGS}}{				
				% \input{\tikzdir/cartoonplots/MoG-unlabeled}
				\input{\tikzdir/GaussianData}
				% \input{../../tikzpics/cartoonplots/GaussianData}
			}{}%
		}
		\subfloat[][]{
			\centering
			\label{subfig:labeledClusters}
			\ifthenelse{\boolean{INCLFIGS}}{				
				% \input{\tikzdir/cartoonplots/MoG-unlabeled}
				\input{\tikzdir/MoG-labeled}
				% \input{../../tikzpics/cartoonplots/MoG-labeled}
			}{}%
		}
		\subfloat[][]{
			\centering
			\label{subfig:unlabeledClusters}
			\ifthenelse{\boolean{INCLFIGS}}{
				% \input{\tikzdir/cartoonplots/MoG-labeled}
				\input{\tikzdir/MoG-unlabeled}
				% \input{../../tikzpics/cartoonplots/MoG-unlabeled}
			}{}%
		}
	\captioning{Simple data sets.}{%
	The data appear to be 
	\subcapref{cluster} normally distributed, or 
	\subcaprefs{labeledClusters}{unlabeledClusters} two-way mixtures of normally distributed data.
	The corresponding learning problems are  
	\subcapref{cluster} density estimation,
	\subcapref{labeledClusters} fitting a fully observed generative model, and
	\subcapref{unlabeledClusters} clustering.
	}
	\label{fig:mixtureOfGaussians}
	\end{figure}
}



\newcommand{\FigSigmoids}{
	\begin{wrapfigure}{r}{0.4\textwidth}
		\newcommand{\figwidth}{1.0\linewidth}%
		\newcommand{\figheight}{1.0\linewidth}%
		\provideboolean{NOLEGEND}%
		\setboolean{NOLEGEND}{true}%
		\ifthenelse{\boolean{INCLFIGS}}{%
			\centering
			% \input{\tikzdir/cartoonplots/sigmoids}
			\input{\tikzdir/sigmoids}
			% \input{../../tikzpics/cartoonplots/sigmoids}
		}{}%
	\captioning{Sigmoidal functions.}{%
	The logistic function (blue) and the Gaussian CDF (green).
	}
	\label{fig:sigmoids}
	\end{wrapfigure}
}


\newcommand{\FigArchitecture}{%
    \begin{figure}
    \def\internode{0.5}%
    \def\interlayer{1.0}%
    \def\numlatent{4}%
    \def\numobserved{6}%
    \pgfmathsetmacro{\offset}{\internode*(\numobserved - \numlatent)/2}%
    \tikzset{%
	    latent/.append style={minimum size=0.2in},
	    obs/.append style={minimum size=0.2in},
	}%
    \subfloat[][]{
		\centering
		\label{subfig:DBNa}
	    \begin{tikzpicture}
	        % Define nodes
	        \foreach \xname / \x in {1,...,\numlatent}{
	        	\pgfmathsetmacro{\xpos}{1.2*(\offset + \x*\internode)}
	        	\node[latent] (x\x) at (\xpos, 0) {};
	        }
	        \pgfmathsetmacro{\xpos}{1.2*(\offset + (\numlatent+1)*\internode)}
	        \node at (\xpos, 0) {$\Generltnts{0}$};


	        \foreach \xname / \x in {1,...,\numobserved}{
	        	\node[obs] (y\x) at (1.2*\x*\internode, -\interlayer) {};
	        }
	        \pgfmathsetmacro{\xpos}{1.2*((\numobserved+1)*\internode)}
	        \node at (\xpos, -\interlayer) {$\Generobsvs{0}$};
	        
	        \foreach \ltntname / \ltntnum in {1,...,\numlatent}{
	        	\foreach \obsvname / \obsvnum in {1,...,\numobserved}{
	        		% \edge[->] {x\ltntnum} {y\obsvnum};
	        		\draw (x\ltntnum) -- (y\obsvnum);
	        	}
	        }

	        \node[minimum height=0.3in] at (1, -3*\interlayer){};
    	\end{tikzpicture}%
    }
    \hfill
    \subfloat[][]{
		\centering
		\label{subfig:DBNb}
	    \begin{tikzpicture}[baseline=(current bounding box.north)]
	        % Define nodes
	        \foreach \xname / \x in {1,...,\numobserved}{
	        	\pgfmathsetmacro{\xpos}{1.2*\x*\internode}
	        	\node[latent] (x\x) at (\xpos, 0) {};

	        	\node[obs] (z\x) at (\xpos, -2*\interlayer) {};
	        }
	        \pgfmathsetmacro{\xpos}{1.2*(\numobserved+1)*\internode}
	        \node at (\xpos, 0) {$\Generobsvs{1}$};
	        \node at (\xpos, -2*\interlayer) {$\Generobsvs{0}$};

	        \foreach \xname / \x in {1,...,\numlatent}{
	        	\pgfmathsetmacro{\xpos}{1.2*(\offset + \x*\internode)}
	        	\node[obs] (y\x) at (\xpos, -\interlayer) {};
	        }
	        \pgfmathsetmacro{\xpos}{1.2*((\numobserved+1)*\internode)}
	        \node at (\xpos, -\interlayer) {$\Generltnts{1}$};

	        \foreach \ltntname / \ltntnum in {1,...,\numlatent}{
	        	\foreach \obsvname / \obsvnum in {1,...,\numobserved}{
	        		% \edge[->] {x\ltntnum} {y\obsvnum};
	        		\draw (x\obsvnum) -- (y\ltntnum);
	        		\draw[-Latex] (y\ltntnum) -- (z\obsvnum) ;
	        	}
	        }

	        \node[minimum height=0.3in] at (1, -3*\interlayer){};
    	\end{tikzpicture}%
    }
    \hfill
    \subfloat[][]{
		\centering
		\label{subfig:DBNc}
	    \begin{tikzpicture}[baseline=(current bounding box.north)]
	        % Define nodes
	        \foreach \xname / \x in {1,...,\numlatent}{
	        	\pgfmathsetmacro{\xpos}{1.2*(\offset + \x*\internode)}
	        	\node[latent] (x\x) at (\xpos, 0) {};
	        	\node[obs] (z\x) at (\xpos, -2*\interlayer) {};
	        }
	        \pgfmathsetmacro{\xpos}{1.2*(\offset + (\numlatent+1)*\internode)}
	        \node at (\xpos, 0) {$\Generltnts{2}$};
	        \node at (\xpos, -2*\interlayer) {$\Generltnts{1}$};

	        \foreach \xname / \x in {1,...,\numobserved}{
	        	\node[obs] (y\x) at (1.2*\x*\internode, -\interlayer) {};
	        	\node[obs] (a\x) at (1.2*\x*\internode, -3*\interlayer) {};
	        }
	        \pgfmathsetmacro{\xpos}{1.2*((\numobserved+1)*\internode)}
	        \node at (\xpos, -\interlayer) {$\Generobsvs{2}$};
	        \node at (\xpos, -3*\interlayer) {$\Generobsvs{0}$};

	        \foreach \ltntname / \ltntnum in {1,...,\numlatent}{
	        	\foreach \obsvname / \obsvnum in {1,...,\numobserved}{
	        		% \edge[->] {x\ltntnum} {y\obsvnum};
	        		\draw (x\ltntnum) -- (y\obsvnum);
	        		\draw (y\obsvnum) -- (z\ltntnum) ;
	        		\draw[-Latex] (z\ltntnum) -- (a\obsvnum) ;
	        	}
	        }
	        		
    	\end{tikzpicture}%
    }

    \captioning{Different views of the exponential family harmonium.}{%
    \subcapref{DBNa} An EFH.
    \subcapref{DBNb} An EFH with one layer ``unrolled.''
    As long as the $\wts{1} = \wts{2}\tr$, this is equivalent to  \subcapref{DBNa}.
    \subcapref{DBNc} An EFH with two layers ``unrolled.''
    }
    \label{fig:architecture}
    \end{figure}
}



\newcommand{\TikzLatentVariableModel}[2]{
	\tikzstyle{factor IPGM}=[factor, fill=none, draw=black]%
	\begin{tikzpicture}
        % Define nodes
        \node[latent] (x) {$\Generltnts$};
        \node[right=0.5cm of x] (xlabel){$\generprior{} = {#1}$};

        \node[obs, below=1.4cm of x] (y) {$\Generobsvs$};
        \node[right=0.5cm of y] (ylabel){$\generemission{} = {#2}$};

        \edge[->] {x} {y};

        \plate{allvars}{(x)(y)}{$N$};
    \end{tikzpicture}% this percent sign is necessary!!
}



\newcommand{\FigFactorAnalyzer}{
	\begin{figure}[!t]	
	\centering
	\subfloat[][]{
		\centering
		\label{subfig:FAimplicit}
		\ifthenelse{\boolean{INCLFIGS}}{
			\TikzLatentVariableModel{\nrml{\vect{0}}{\mat{I}}}{\nrml{\EMISSIONWTS\argltnts + \emissionwts}{\diagonalMat}}
		}{}%
	}
	\hspace{0.1in}
	\subfloat[][]{
		\centering
		\label{subfig:FAexplicit}
		\ifthenelse{\boolean{INCLFIGS}}{
			\tikzstyle{factor IPGM}=[factor, fill=none, draw=black]%
		    \begin{tikzpicture}
		        % Define nodes
		        \node[latent] (x1) {$\Generltnt{1}$};
		        \node[latent, right=0.5cm of x1] (x2) {$\Generltnt{2}$};
		        \node[latent, right=0.5cm of x2] (x3) {$\Generltnt{3}$};

		        \node[obs, below=1.4cm of x1] (y2) {$\Generobsv{2}$};
		        \node[obs, left=0.5cm of y2] (y1) {$\Generobsv{1}$};
		        \node[obs, right=0.5cm of y2] (y3) {$\Generobsv{3}$};
		        \node[obs, right=0.5cm of y3] (y4) {$\Generobsv{4}$};
		        \node[obs, right=0.5cm of y4] (y5) {$\Generobsv{5}$};
		        
		        \edge[->] {x1,x2,x3} {y1,y2,y3,y4,y5};
		        
		        \plate{allvars}{(x1)(x2)(x3)(y1)(y2)(y3)(y4)(y5)}{$N$};
		    \end{tikzpicture}% this percent sign is necessary!!
		}{}%
	}
	\captioning{The factor analyzer.}{%
	\subcapref{FAimplicit} The most abstract version of the model (cf.\ the GMM in \fig{GMM}).
	\subcapref{FAexplicit} The independence statements made explicit.
	}\label{fig:FA}
	\end{figure}
}



\newcommand{\FigSparseCodingModel}{
	\begin{figure}[!t]	
	\centering
	\subfloat[][]{
		\centering
		\label{subfig:SCimplicit}
		\ifthenelse{\boolean{INCLFIGS}}{
			\TikzLatentVariableModel{%
				\frac{1}{Z}\prod_{k=1}^{K}\expop{-\energy(\argltnt{k})}%
			}{%
				\nrml{\EMISSIONWTS\argltnts}{\frac{1}{\lambda}\mat{I}}%
			}
		}{}%
	}
	\hspace{0.1in}
	\subfloat[][]{
		\centering
		\label{subfig:SCexplicit}
		\ifthenelse{\boolean{INCLFIGS}}{
			\tikzstyle{factor IPGM}=[factor, fill=none, draw=black]%
		    \begin{tikzpicture}
		        % Define nodes
		        \node[latent] (x1) {$\Generltnt{1}$};
		        \node[latent, right=0.5cm of x1] (x2) {$\Generltnt{2}$};
		        \node[latent, right=0.5cm of x2] (x3) {$\Generltnt{3}$};
		        \node[latent, right=0.5cm of x3] (x4) {$\Generltnt{4}$};
		        \node[latent, right=0.5cm of x4] (x5) {$\Generltnt{5}$};

		        \node[obs, below=1.4cm of x2] (y1) {$\Generobsv{1}$};
		        \node[obs, right=0.5cm of y1] (y2) {$\Generobsv{1}$};
		        \node[obs, right=0.5cm of y2] (y3) {$\Generobsv{3}$};
		        
		        \edge[->] {x1,x2,x3,x4,x5} {y1,y2,y3};
		        
		        \plate{allvars}{(x1)(x2)(x3)(x4)(x5)(y1)(y2)(y3)}{$N$};
		    \end{tikzpicture}% this percent sign is necessary!!
		}{}%
	}
	\captioning{A sparse-coding model.}{%
	\subcapref{SCimplicit} The most abstract version of the model (cf.\ the GMM in \fig{GMM} and the factor analyzer in \protect\subfig{FAimplicit}).
	The energy function $\energy$ enforces sparseness; e.g.,
	$\energy(\protect\argltnt{k}) = \alpha_k\absop{\protect\argltnt{k}}$,
	or
	$\energy(\protect\argltnt{k}) = \logop{\beta^2 + \protect\argltnt{k}^2}$
	\subcapref{SCexplicit} The independence statements and overcompleteness made explicit.
	}\label{fig:SC}
	\end{figure}
}




\newcommand{\FigSimplePGM}{
	\begin{figure}[!t]	
	\centering
	\subfloat[][]{
		\centering
		\label{subfig:EmissionSourceModelForward}
		\ifthenelse{\boolean{INCLFIGS}}{
			\begin{tikzpicture}
				% Define nodes
				\node[latent] 	(source){$\Generltnts$};
				\node[latent, below=1.5cm of source] 	(emission){$\Generobsvs$};
				
				\node[right=0cm of source]	(prior){$\generprior{} = \nrml{\vect{\mu}_{\generltntvar}}{\mat{\Sigma}_{\generltntvar}}$};
				\node[right=0cm of emission]							(likelihood){$\generemission{} = \nrml{\vect{\mu}_{\generobsvvar|\generltntvar}}{\mat{\Sigma}_{\generobsvvar|\generltntvar}}$};
				
				\edge {source} {emission}; 
			\end{tikzpicture}
		}{}
	}
	\hspace{0.5in}
	\subfloat[][]{
		\centering
		\label{subfig:EmissionSourceModelReverse}
		\ifthenelse{\boolean{INCLFIGS}}{
			\begin{tikzpicture}
				% Define nodes
				\node[latent] 						(source){$\Generltnts$};
				\node[latent, below=1.5cm of source] 	(emission){$\Generobsvs$};
				
				\node[right=0cm of source]								(likelihood){$\generposterior{} = \nrml{\vect{\mu}_{\generltntvar|\generobsvvar}}{\mat{\Sigma}_{\generltntvar|\generobsvvar}}$};
				\node[right=0cm of emission]	(prior){$\genermarginal{} = \nrml{\vect{\mu}_{\generobsvvar}}{\mat{\Sigma}_{\generobsvvar}}$};
				
				\edge {emission} {source}; 
			\end{tikzpicture}
		}{}
	}
	\captioning{Emission and source.}{These models make equivalent independence statements about $\protect\Generltnts$ and $\protect\Generobsvs$, but parameterize the distribution differently.}\label{fig:EmissionSourceModel}
	\end{figure}
}






\newcommand{\FigHMM}{%
	\providecommand\suffix{}
    \begin{figure}[!t]
		% \resizebox{1.0\textwidth}{!}{
		\ifthenelse{\boolean{INCLFIGS}}{%
			\providecommand\PGMorientation{180}%
			\providecommand\thisTikzPicScale{0.8}%
			\providecommand\PGMmirror{1.0}%
			\providecommand\InputSequenceLength{7}%
			\providecommand\initialtime{1}%
			\provideboolean{SHOW_OBSVS}%
			\setboolean{SHOW_OBSVS}{true}%
			\input{\tikzdir/HMM}%
		}{}
		%}
    \captioning{The hidden Markov Model.}{%
    Generally, this name is used only if the latent state is discrete, but the same architecture underlies state-space models with real-valued hidden states.
	}\label{fig:HMM\suffix}
	\end{figure}
}



\newcommand{\FigFilterSmootherFragments}{
	\providecommand{\timevar}{n}
	\begin{figure}[!t]	
	\centering
	\subfloat[][]{%
		\centering%
		\label{subfig:filterTransition}%
		\ifthenelse{\boolean{INCLFIGS}}{%
			\begin{tikzpicture}

				% vertices
				\node[latent](state){$\Generltntsprev$};
				\node[latent,right=1.5cm of state](emission){$\Generltntsnow$};
				
				% their labels
				\node[%
					above=0cm of state,%
					align=right,%
					execute at begin node=\setlength{\baselineskip}{3.5ex},%
				](stateprior){$\filter{index=\timevar-1} $};
				\node[%
					below=0cm of emission,%
					align=right,%
					execute at begin node=\setlength{\baselineskip}{3.5ex},%
				](likelihood){$\genertransition{} $};
				
				\edge {state} {emission}; 
			\end{tikzpicture}%
		}{}
	}
	\subfloat[][]{%
		\centering%
		\label{subfig:filterlookaheadEmission}%
		\ifthenelse{\boolean{INCLFIGS}}{%
			\begin{tikzpicture}
				
				% vertices
				\node[latent,](state){$\Generltntsnow$};
				\node[obs,below=1.5cm of state,minimum size=1cm](emission){$\Generobsvsnow$};
				
				% their labels
				\node[%
					above=0cm of state,%
				](prior){$\filtertimeupdated{} $};
				\node[%
					below=0cm of emission,%
					align=right,%
					execute at begin node=\setlength{\baselineskip}{3.5ex},%
				](likelihood){$\generemission{patent=\dataobsvs{\index},index=\timevar} $};
				
				\edge {state} {emission}; 
			\end{tikzpicture}%
		}{}
	}
	\subfloat[][]{%
		\centering%
		\label{subfig:smootherFutureconditioned}%
		\ifthenelse{\boolean{INCLFIGS}}{%
			\begin{tikzpicture}
				
				% vertices
				\node[latent](state){$\Generltntsnow$};
				\node[latent,left=1.5cm of state](emission){$\Generltntsprev$};
				
				% their labels
				\node[%
					above=0cm of state,%
				](prior){$\smoother{} $};
				\node[%
					below=0cm of emission,%
					align=right,%
					execute at begin node=\setlength{\baselineskip}{3.5ex},%
				](likelihood){$\generreversetransition{paramdisplay={,\dataobsvsalltime}} $};
				
				\edge {state} {emission}; 
			\end{tikzpicture}%
		}{}
	}
	\captioning{Three graphical model fragments for HMM inference problems.}{
		The various inference problems for HMM-like models can be expressed in terms of recursive application to these three fragments of two operations: marginalizing out the source variable (\emph{marginalization}) and computing the posterior distribution (\emph{inversion}).
 		\subcapref{filterTransition}
 		Marginalization:\ the time update.
 		Inversion:\ future conditioning.
 		\subcapref{filterlookaheadEmission}
 		Marginalization:\ the recursion for the data marginal.
 		Inversion:\ the measurement update.
 		\subcapref{smootherFutureconditioned}
 		Marginalization:\ the backward step.
 		Inversion:\ the recursion for the posterior distribution over sequences.
		The distributions have been written in terms of a particular instantiation of the observations to emphasize their use in \emph{inference}.
	}\label{fig:FilterSmootherFragments}
	\end{figure}
}





\newcommand{\FigICA}{
	\begin{figure}[!t]	
	\centering
	\vtop{%
		\subfloat[][]{%
			\label{subfig:ICAgenerativemodel}%
			\ifthenelse{\boolean{INCLFIGS}}{%
				\def\Nltnt{4}%
				\def\Nobsv{4}%
				\def\emissionmatrix{\EMISSIONWTS}%
				\input{tikz/GM_LatentCauses}%
			}{}%
		}%
		\hfill
		\subfloat[][]{%
			\label{subfig:ICAdiscriminativemodel}%
			\ifthenelse{\boolean{INCLFIGS}}{%
				\def\inputs{\Generobsv}%
				\def\mixed{\Generltnt}%
				\def\outputs{\Generaux}%
				\def\weight{\recogwt}%
				\def\Nneuronssym{\Ncat}%
				\input{\tikzdir/NN_ICA}%
			}{}%
		}%
	}
	\captioning{``Infomax'' independent-components analysis.}{
	\subcapref{ICAgenerativemodel} The generative model.
	\subcapref{ICAdiscriminativemodel} The discriminative model.
	Note that $\protect\EMISSIONWTS = \protect\RECOGWTS^{-1}$.
	}\label{fig:ICA}
	\end{figure}
}




\newcommand{\FigPerceptrons}{
	\begin{figure}[!t]	
		\ifthenelse{\boolean{INCLFIGS}}{%
			\def\inputs{\Generobsv}%
			\def\mixed{\Generltnt}%
			\def\outputs{\Generaux}%
			\def\weight{\recogwt}%
			\def\Nneuronssym{\Ncat}%
			\input{\tikzdir/NN_ICA}%
		}{}%
	\captioning{A square neural network.}{}\label{fig:perceptrons}
	\end{figure}
}



\newcommand{\FigTikzTwoMarkovChains}{
	\begin{figure}[!ht]	
		\centering
		\subfloat[][]{
			\label{subfig:XYZmarkovChain}
			\ifthenelse{\boolean{INCLFIGS}}{
				\def\yrtikzMCx{$\Stims$}
				\def\yrtikzMCy{$\Obsvs$}
				\def\yrtikzMCz{$\Suffstats{}$}
				\input{tikz/MarkovChain.tex}
			}{}
		}\hspace{0.1in}
		\subfloat[][]{
			\label{subfig:XZYmarkovChain}
			\ifthenelse{\boolean{INCLFIGS}}{
				\def\yrtikzMCx{$\Stims$}
				\def\yrtikzMCy{$\Suffstats{}$}
				\def\yrtikzMCz{$\Obsvs$}
				\input{tikz/MarkovChain.tex}
			}{}
		}
		\captioning{Two Markov chains.}{
			\subcapref{XYZmarkovChain} $\protect\Stims$ and $\protect\Suffstats{}$ are conditionally independent given $\protect\Obsvs$.
			\subcapref{XZYmarkovChain} $\protect\Stims$ and $\protect\Obsvs$ are conditionally independent given $\protect\Suffstats{}$.
		}\label{fig:twoMarkovChains}
	\end{figure}
}



\newcommand{\FigKindsOfMatrices}{
	\begin{figure}[ht!]
		\centering
			\ifthenelse{\boolean{INCLFIGS}}{
				\input{\tikzdir/KindsOfMatrices.tex}
			}{}
		\captioning{A taxonomy of matrices.}{}\label{kindsOfMatrices}
	\end{figure}
}



\newcommand{\FigMixedModel}{
	\begin{figure}[!t]	
	\centering
	\subfloat[][]{
		\centering
		\label{subfig:unnormalizedMRF}
		\ifthenelse{\boolean{INCLFIGS}}{
			\begin{tikzpicture}
				% Define nodes
				\node[latent] 	(X1){$\Generltnts{1}$};
				\node[latent, below=1.5cm of X1] 	(X2){$\Generltnts{2}$};
				\node[latent, right=1.5cm of X1] 	(X3){$\Generltnts{3}$};
				\node[latent, right=1.5cm of X2] 	(X4){$\Generltnts{4}$};
								
				\edge[-] {X1} {X2,X3}; 
				\edge[-] {X4} {X2,X3}; 
			\end{tikzpicture}
		}{}
	}
	\hspace{0.5in}
	\subfloat[][]{
		\centering
		\label{subfig:normalizedMRF}
		\ifthenelse{\boolean{INCLFIGS}}{
			\begin{tikzpicture}
				% Define nodes
				\node[latent] 	(X1){$\Generltnts{1}$};
				\node[latent, below=1.5cm of X1] 	(X2){$\Generltnts{2}$};
				\node[latent, right=1.5cm of X1] 	(X3){$\Generltnts{3}$};
				\node[latent, right=1.5cm of X2] 	(X4){$\Generltnts{4}$};

				\node[obs, below right=0.5cm and 1.5cm of X3] 	(Z){$\Generobsvs{}$};				
								
				\edge[-] {X1} {X2,X3}; 
				\edge[-] {X4} {X2,X3}; 
				\edge[-] {Z}{X1,X2,X3,X4}; 
			\end{tikzpicture}
		}{}
	}
	\captioning{Alternative interpretation of undirected model.}{The unnormalized distribution represented by the product of potentials in \subcapref{unnormalizedMRF} corresponds to a slice through the normalized distribution represented by the graph in \subcapref{normalizedMRF}.}\label{fig:mixedModel}
	\end{figure}
}



\newcommand{\FigBitsBack}{
	\begin{figure}[!ht]
	\scriptsize%
	\centering%
	\tikzset{var/.style={minimum width=0.25in, draw=none}}
	\tikzset{coder/.style={trapezium,trapezium angle=70,trapezium stretches=true,draw=black,minimum width=0.7in,minimum height=0.35in}}
	\tikzset{decoder/.style={coder,shape border rotate=0}}
	\tikzset{encoder/.style={coder,shape border rotate=180}}
	% https://tex.stackexchange.com/questions/494953
	\tikzset{prior/.style={rectangle,rounded corners,draw=black,minimum width=0.5in,minimum height=0.35in}}
	\tikzset{diff/.style = {
		circle, draw, minimum size=0.3in,
	    append after command={\pgfextra{\let\LN\tikzlastnode}
	        node[left]     at (\LN.center) {$-$}
	        node[above]    at (\LN.center) {$+$}
		},
	}}
	\tikzset{sum/.style = {
		circle, draw, minimum size=0.3in,
	    append after command={\pgfextra{\let\LN\tikzlastnode}
	        node[left]     at (\LN.center) {$+$}
	        node[above]    at (\LN.center) {$+$}
		},
	}}
	\begin{tikzpicture}[node distance=1cm, auto]
	    \scriptsize
	    \tikzset{>={latex}}

	    % SENDER
	    \node[var](extraS){$\Dataauxs{}$};
	    \node[encoder,right=0.25in of extraS](encoderS){$\recogposterior{} $};
	    \node[var,below=0.25in of encoderS](ltntS){$\Recogltnts$};
	    \node[decoder, below=0.25in of ltntS](decoderS){$\generemission{} $};
	    \node[var,below=0.25in of decoderS](error){$\vect{E}$};
		\node[var,above=0.25in of encoderS](obsvS){$\Dataobsvs$};
		\node[right=0.25in of obsvS](A){};
	    \node[prior, right=0.5in of ltntS](priorS){$\generprior{} $};

	    \draw[->,thick] (extraS) -- (encoderS);
	    \draw[->,thick] (obsvS) -- (encoderS);
	    \draw[->,thick,decorate,decoration=snake] (encoderS) -- (ltntS);
	    \draw[->,thick] (ltntS) -- (decoderS);
	    \draw[->,thick] (decoderS) -- (error);
	    \draw[thick] (obsvS) -- (A.center);
	    \draw[->,thick] (A.center) |- (decoderS);
	    \draw[->,thick] (ltntS) -- (priorS);

	    \node[
	    	draw=Set2-A,ultra thick,solid,rounded corners,
	    	fit=
	    		(encoderS.bottom right corner)
	    		(priorS.east |- decoderS.south),
	    	label={[color=black,above right]{sender}}
	    ] (sender) {};


	    
	    % RECEIVER
	    \node[prior, right=0.5in of priorS](priorR){$\generprior{} $};
	    \node[var, right=0.25in of priorR](ltntR){$\Recogltnts{} $};
	    \node[encoder,above=0.25in of ltntR](encoderR){$\recogposterior{} $};
	    \node[decoder] at (encoderR |- decoderS) (decoderR){$\generemission{} $};
	    \node[var,right=0.45in of encoderR](extraR){$\Dataauxs{} $};
	    \node[var,right=0.2in of decoderR](obsvR){$\Dataobsvs{} $};

	    \node (C) at (obsvR |- obsvS){};

	    \draw[->,thick] (priorS) -- (priorR);
	    \draw[->,thick] (priorR) -- (ltntR);
	    \draw[->,thick] (ltntR) -- (decoderR);
	    \draw[->,thick] (ltntR) -- (encoderR);
	    \draw[->,thick] (error) -| (decoderR);
	    \draw[->,thick] (decoderR) -- (obsvR);
	    \draw[->,thick] (encoderR) -- (extraR);
	    \draw[->,thick] (obsvR) -- (C.center) -| (encoderR);

		\node[
	    	draw=Set2-B,ultra thick,solid,rounded corners,
	    	fit=
	    		(priorR.west |- encoderR.north)
	    		(decoderR.bottom right corner)
	    	,
	    	label={[color=black,above]{receiver}}
	    ] (receiver) {};

	\end{tikzpicture}%
	\captioning{The bits-back procedure.}{The sender (left) stochastically encodes observations $\protect\Dataobsvs{}$ into latent codes $\protect\Recogltnts{}$ with the recognition model $\protect\recogposterior{} $, with the randomness provided by some ``extra bits'' $\protect\Dataauxs{}$.
	Under any generative model $\protect\generemission{} $, $\protect\Dataobsvs{}$ cannot be reconstructed from $\protect\Recogltnts{}$ without some error, $\vect{E}$.
	The sender encodes these errors (with $\protect\generemission{} $) and transmits them to the receiver.
	The latent codes are likewise approximately uniformized, in this case with the generative prior $\protect\generprior{} $, and transmitted to the receiver.
	The receiver (right) in turn transforms these messages back into latent codes (again with the generative prior), and uses these along with the error terms to reconstruct $\protect\Dataobsvs{}$ (using $\protect\generemission{} $).
	She then proceeds to use the reconstructed $\protect\Dataobsvs{}$, along with the latent codes $\protect\Recogltnts{}$, to recover the ``extra bits,'' $\protect\Dataauxs{}$.
	}
	\end{figure}
}




\newcommand{\FigNCEgeneralizationsPGMs}{
	\begin{figure}[!h]	
	\centering
	\subfloat[][]{
		\centering
		\label{subfig:InfoNCE}
		\ifthenelse{\boolean{INCLFIGS}}{
			\tikzstyle{factor IPGM}=[factor, fill=none, draw=black]%
			\begin{tikzpicture}
		        % Define nodes
		        \node[latent] (x) {$\Generltnts$};
		        \node[right=0.5cm of x] (xlabel){$\generprior{paramdisplay={}} = \frac{1}{\Ncat}$};

		        \node[obs, below=1.4cm of x] (y) {$\Generobsvs{}$};
		        \node[right=0.5cm of y] (ylabel){$\generemission{} = \genermarginalunnormalized{} ^{\argltnt{\ncat}}\datanoisemarginal{patent=\argobsvs{}} ^{1 - \argltnt{\ncat}}$};

		        \edge[->] {x} {y};

		        \plate{observations}{(y)}{$\Ncat$};
		        \plate{allvars}{(x)(y)(observations)}{$\Samplevar$};
		    \end{tikzpicture}% this percent sign is necessary!!
		}{}%
	}
	\subfloat[][]{
		\centering
		\label{subfig:localNCE}
		\ifthenelse{\boolean{INCLFIGS}}{
			\tikzstyle{factor IPGM}=[factor, fill=none, draw=black]%
			\begin{tikzpicture}
		        % Define nodes
		        \node[latent] (x) {$\Generltnts$};
		        \node[right=0.5cm of x] (xlabel){$\generprior{paramdisplay={}} = \left(\frac{1}{2}\right)^{\Ncat}$};

		        \node[obs, below=1.4cm of x] (y) {$\Generobsvs{}s$};
		        \node[right=0.5cm of y] (ylabel){$\generemission{} = \prod_{\ncat=1}^{\Ncat}\genermarginalunnormalized{patent=\argobsv{\ncat}} ^{\argltnt{\ncat}}\datanoisemarginal{patent=\argobsv{k}} ^{1 - \argltnt{\ncat}}$};

		        \edge[->] {x} {y};

		        \plate{observations}{(x)(y)}{$\Ncat$};
		        \plate{allvars}{(x)(y)(observations)}{$\Samplevar$};
		    \end{tikzpicture}% this percent sign is necessary!!
		}{}%
	}
    \captioning{Generalizations of NCE for representation learning.}{%
    \subcapref{InfoNCE} InfoNCE.
    For each toss of a $\protect\Ncat$-sided die, $\protect\Generltnts{}$, one sample (corresponding to the face of the die that came up) is drawn from the model distribution, and $\protect\Ncat-1$ samples are drawn from a noise distribution.
    \subcapref{localNCE} ``Local NCE'' (as in {\sc wav2vec}).
    For each of $\protect\Samplevar$ trials, a coin is flipped $\protect\Ncat$ times to determine whether to draw data from the model distribution or a noise distribution.
    Note that the \emph{data} distribution is the same for both models, and corresponds to \subcapref{InfoNCE}, with $\protect\genermarginalunnormalized{} $ replaced by the data (\eqn{InfoNCEdatadistribution}).
    }\label{fig:NCEgeneralizationsPGMs}
	\end{figure}
}

%-----------------------------------------------------------------------------%
% ###END
%-----------------------------------------------------------------------------%






==> stys/defaultPreamble.tex <==
% Standard figure/caption setup and standard packages.  In contrast, jgmstd
%  contains the standard *macros*.  The only reason not to merge the two is
%  that some of these packages might conflict withjournal requirements, whereas 
%  jgmstd.sty imports the bare minimum packages required to define its macros.

%-------------------------EXPECTED TO BE DEFINED OUTSIDE----------------------%
\providecommand{\stydir}{../stys}
\providecommand{\bibsdir}{../bibs}
\providecommand{\tikzdir}{../tikzpics}
%-----------------------------------------------------------------------------%


%-------------------------------DEFAULT PACKAGES------------------------------%
\usepackage{%
	amsmath,amsfonts,amssymb,amsthm,
	graphicx,rotating,booktabs,
	versions,ifthen,siunitx,bbm,
	%%%%%%
	% temporarily removed for NIPS, AAAI
	% geometry
	%%%%%%
}
% \usepackage[table]{xcolor}
% \usepackage{xcolor}
\usepackage[dvipsnames]{xcolor}
\usepackage{pgf,tikz,pgfplots} 
% \usepackage{mathpazo}
\usetikzlibrary{%
 	positioning,calc,patterns,shapes,arrows,intersections,backgrounds,fit,shadings,decorations.text,shadows,fadings,bayesnet,arrows.meta,spy
}
\usepgfplotslibrary{colorbrewer,colormaps,fillbetween,groupplots}

% For compatibility with latexml, which would be unhappy when it fails to
%  find "bindings" for jgmstd loaded as \usepackage{\stydir/jgmstd}.
\ifdefined\matttlderiv
	% do nothing
\else
	\makeatletter
	\input{\stydir/jgmstd.sty}
	\makeatother
\fi
%-----------------------------------------------------------------------------%


%------------------------------- FIGURE SETUP --------------------------------%
\newboolean{INCLFIGS} % default is false
\setboolean{INCLFIGS}{true}

% caption and subfigure settings
% \usepackage{caption,subfig}
\usepackage{subcaption}
\newcommand{\captioning}[2]{\caption{{\bf #1} {#2}}}
% \renewcommand{\captioning}[2]{}
\captionsetup{font={small}}
% see ucsf/Edgefield/figures.tex for other useful captionsetup options
\renewcommand{\thesubfigure}{\Alph{subfigure}}

% if there're no figures, don't put subfigure letters on the blank spaces where
%  the figures would be (labelformat=empty)
\ifthenelse{\boolean{INCLFIGS}}{
% 		\usepackage[scaled]{uarial}
% 		\usepackage[T1]{fontenc}
% 		\usepackage[utf8]{inputenc}
% 		\DeclareCaptionFont{caca}{\fontfamily{fvs}\fontseries{b}\selectfont}
% 		\captionsetup[subfloat]{font={large,sf,caca},labelformat=simple,labelsep=none}
	\captionsetup[subfloat]{font={Large,sf},labelformat=simple,labelsep=none}
}{
	\captionsetup[subfloat]{labelformat=empty,labelsep=none}
}
%-----------------------------------------------------------------------------%


%--------------------------------- COLOR -------------------------------------%
\newcommand{\colorprovide}[2]{\@ifundefinedcolor{#1}{\colorlet{#1}{#2}}{}}
%-----------------------------------------------------------------------------%


%-------------------------------DIRECTORIES-----------------------------------%
% \catcode`\#=12\def\hashsign{#}\catcode`\#=6
% \newcommand{\cartoonplots}{\tikzdir/\hashsign cartoonplots}
\newcommand{\cartoonplots}{\tikzdir/cartoonplots}
\newcommand{\dataplots}{\tikzdir/dataplots}
\newcommand{\graphicalmodels}{\tikzdir/graphicalmodels}
\newcommand{\illustrativeplots}{\tikzdir/illustrativeplots}
\newcommand{\kinematicchains}{\tikzdir/kinematicchains}
\newcommand{\OPP}{\tikzdir/OPP}
%-----------------------------------------------------------------------------%
